Deterministic Function Computation with Chemical Reaction Networks

Chemical reaction networks (CRNs) formally model chemistry in a well-mixed solution. CRNs are widely used to describe information processing occurring in natural cellular regulatory networks, and with upcoming advances in synthetic biology, CRNs are a promising language for the design of artificial molecular control circuitry. Nonetheless, despite the widespread use of CRNs in the natural sciences, the range of computational behaviors exhibited by CRNs is not well understood. CRNs have been shown to be efficiently Turing-universal when allowing for a small probability of error. CRNs that are guaranteed to converge on a correct answer, on the other hand, have been shown to decide only the semilinear predicates. We introduce the notion of function, rather than predicate, computation by representing the output of a function f:N^k --> N^l by a count of some molecular species, i.e., if the CRN starts with n_1,...,n_k molecules of some "input" species X1,...,Xk, the CRN is guaranteed to converge to having f(n_1,...,n_k) molecules of the "output" species Y1,...,Yl. We show that a function f:N^k --> N^l is deterministically computed by a CRN if and only if its graph {(x,y) | f(x) = y} is a semilinear set. Furthermore, each semilinear function f can be computed on input x in expected time O(polylog(|x|)).

==> SystematicExample_latex.tex <==
X_1 \rxn X_1^1 + X_1^2 + X_1^3 \\
X_2 \rxn X_2^1 + X_2^2 + X_2^3 \\


& X_1^1 \rxn P^1 + P^1  \\
& X_2^1 \rxn C^1  \\
& X_2^2 \rxn P^2


X_2^3 + L^0 \rxn L^1 \\
X_1^3 + L^1 \rxn L^0



L^1 + Y + C^1   \rxn   L^1 + \hat{C}^1  \\
L^1 + P^1   \rxn   L^1 + Y + \hat{P}^1  \\
%
L^1 + Y + \hat{P}^2   \rxn   L^1 + P^2  \\
%
%
L^0 + \hat{C}^1   \rxn   L^0 + Y + C^1  \\
L^0 + Y + \hat{P}^2 \rxn   L^0 + P^2  \\
%
L^0 + P^2   \rxn   L^0 + Y + \hat{P}^2  



==> dfccrn.tex <==
\input{main}

==> func-speed_ds_old.tex <==
\section{Speed of deterministic function computation}
\label{sec:detfuncspeed}


\repds{}{Lemma~\ref{lem-pres-comp} describes how a CRN can deterministically compute any semilinear function.
There are two problems with this construction.
First, we assumed the fairness condition; however, it is not always true that an infinite execution sequence in the kinetic model will be fair with probability 1 if the state space is unbounded (as in our construction).
Second, the particular construction we employed relied on a random search for the correct output. 
It can be shown that its instantiation in the kinetic model would require expected time at least exponential (in the number of molecules), like the predicate-deciding CRDs of~\cite{AngluinAE06}.
Angluin, Aspnes, and Eisenstat combined the results of \cite{AngluinAE06} with a fast, error-prone simulation of a bounded-space Turing machine to show that semilinear predicates can be computed without error in expected polylogarithmic time~\cite{angluin2006fast}.
In this section we show that a similar technique implies that semilinear functions can be computed by CRNs without error in expected polylogarithmic time in the kinetic model.}

\opt{normal}{
For our asymptotic time analysis, let $n =  \|\vx\|$.
In this section, the total molecular count attainable will always be $O(n)$;
thus, for by finite density constraint, the volume $v = O(n)$.
}

\input{thm-4-1}


\begin{lem} \label{lem-compute-semilinear-n-log-n}
  Let $f:\N^k\to\N^l$ be semilinear.  Then there is a CRC $\calC$ that stably computes $f$, and the expected time for $\calC$ to reach a count-stable configuration on input $\vx$ is $O(\|\vx\| \log \|\vx\|)$ (where the $O()$ constant depends on $f$).
\end{lem}


\opt{submission}{
A proof of Lemma~\ref{lem-compute-semilinear-n-log-n} is proved in the technical appendix.
Intuitively, it works as follows.
Any semilinear function $f$ can be expressed as a union of affine partial functions $f_1,\ldots,f_p$.
Each of these can be computed by a CRC that produces its output molecules monotonically in $O(n \log n)$ time, where $n = \|\vx\|$.
Furthermore, each point $\vx$ in the domain of $f$ can be tested by a semilinear predicate to see which is the first $f_i$ in the list whose domain contains $\vx$.
All functions $f_i$ are computed at once by parallel CRCs, but in the end only one's output is activated, and the others are deactivated, according to the semilinear predicate that eventually indicates which function to use (also in time $O(n \log n)$).
}


\newcommand{\proofTechnicalLemmas}{
\begin{proof}\opt{submission}{[of Lemma~\ref{lem-compute-semilinear-n-log-n}]}
  By Lemma~\ref{lem-pres-comp}, there is a CRC $\calC_s$ that stably computes $f$.
  However, that CRC is too slow to use in this proof.
  We provide an alternative proof that every semilinear function can be computed by a CRC in expected time $O(\|\vx\| \log \|\vx\|)$.
  Rather than relying on a random search of the output space as in Lemma~\ref{lem-pres-comp}, it computes the function more directly.
  
\opt{submission}{Let $n =  \|\vx\|$.
In this section, the total molecular count attainable will always be $O(n)$;
thus, for by finite density constraint, the volume $v = O(n)$.}  

  By Lemma~\ref{lem-semilinear-function-finite-union-linear}, there is a finite set $F=\{f_1:\N^k \dashrightarrow \N^l,\ldots,f_m:\N^k \dashrightarrow \N^l\}$ of affine partial functions, where each $\dom f_i$ is a linear set, such that, for each $\vx\in\N^k$, if $f_i(\vx)$ is defined, then $f(\vx)=f_i(\vx)$.
  We compute $f$ on input $\vx$ as follows.
  Since each $\dom f_i$ is a linear (and therefore semilinear) set, we compute each predicate $\phi_i = $ ``$\vx \in \dom f_i$ and $(\forall 1 \leq i' < i)\ \vx \not\in \dom f_{i'}$?'' by separate parallel CRD's.
  (The latter condition ensures that for each $\vx$, precisely one of the predicates is true.)

  By Lemma~\ref{lem-compute-linear-fast}, we can compute each $f_i$ by parallel CRC's.
  Assume that for each $1 \leq i \leq m$ and each $1 \leq j \leq l$, the $j$th output of the $i$th function is represented by species $\hY^i_j$.
  Each $\hY^i_j$ is an ``inactive'' version of ``active'' output species $Y^i_j$.

  For each $1 \leq i \leq m$, we assume that the CRD computing the predicate $\phi_i$ represents its output by voting species $L^i_1$ to represent ``yes'' and $L^i_0$ to represent ``no''.
  Then add the following reactions for each $1 \leq i \leq m$ and each $1 \leq j \leq l$:
  \begin{eqnarray*}
    L^i_1 + \hY^i_j &\to& L^i_1 + Y^i_j + Y_j
    \\
    L^i_0 + Y^i_j &\to& M^{i}_{j} \\
    M^{i}_{j} + Y_j &\to& L^i_0 + \hY^i_j.
  \end{eqnarray*}
  That is, a ``yes'' answer for function $i$ activates the $i$th output and a ``no'' answer deactivates the $i$th output.
  Eventually each CRD stabilizes so that precisely one $i$ has $L^i_1$ present, and for all $i' \neq i$, $L^{i'}_0$ is present.
  At this point, all outputs for the correct function $f_i$ are activated and all other outputs are deactivated.
  Since eventually the count of $Y_j^i$ stabilizes to 0 for all but one value of $i$, this ensures that $\# Y_j$ stabilizes to the correct value of output $\vy_j$.

  It remains to analyze the expected time to stabilization.
  Let $n = \|\vx\|$.
  By Lemma~\ref{lem-compute-linear-fast}, the expected time for each affine function computation to complete is $O(n \log n)$.
  %Since the CRC used in Lemma~\ref{lem-compute-linear-fast} monotonically produces $\hY_i^j$, by the choice of reactions above, the total molecular count is bounded by $O(n)$, so the same volume is required.
  Since the $\hY_i^j$ are produced monotonically, the most $Y_i^j$ molecules that are ever produced is $\#_\infty \hY_i^j$.
  Since %the tail decays exponentially, and
we have $m$ computations in parallel, the expected time for all of them to complete is $O((n \log n) m) = O(n \log n)$ (since $m$ depends on $f$ but not $n$).
  We must also wait for each predicate computation to complete.
  By Theorem 5 of~\cite{AngluinAE06}, each of these predicates takes expected time $O(n)$ to complete, so all of them complete in expected time $O(n m) = O(n)$.

  At this point, the $L^i_1$ leaders must convert inactive output species to active, and $L^{i'}_0$ (for $i' \neq i$) must convert active output species to inactive.
  A similar analysis to the proof of Lemma~\ref{lem-compute-linear-fast} shows that each of these requires at most $O(n \log n)$ expected time, therefore they all complete in expected time $O((n \log n) m) = O(n \log n)$.
\qedl\end{proof}


\begin{lem}\label{lem-semilinear-function-finite-union-linear}
  Let $f:\N^k\to\N^l$ be a semilinear function.
  Then there is a finite set $\{f_1:\N^k \dashrightarrow \N^l,\ldots,f_m:\N^k \dashrightarrow \N^l\}$ of affine partial functions, where each $\dom f_i$ is a linear set, such that, for each $\vx\in\N^k$, if $f_i(\vx)$ is defined, then $f(\vx)=f_i(\vx)$.
\end{lem}


\begin{proof}
  Let
  $
    F = \setl{ (\vx,\vy) \in \N^k \times \N^l }{ f(\vx) = \vy }
  $
  be the graph of $f$.
  Since $F$ is semilinear, it is a finite union of linear sets $\{L_1,\ldots,L_n\}$.
  It suffices to show that each of these linear sets $L_m$ is the graph of an affine partial function.
  Let $L'_m$ be the $(k+1)$-dimensional projection of $L_m$ onto the coordinates defined by $\vx$ and $\vy_i$, which is linear because $L_m$ is.
  Since $L'_m$ is linear, there exist vectors $\vec{b},\vec{u}^1,\ldots,\vec{u}^p \in\N^{k+1}$ such that $L'_m=\setl{\vec{b} + n_1 \vec{u}^1 + \ldots + n_p \vec{u}^p}{n_1,\ldots,n_p\in\N}.$
  %We consider each output coordinate separately, since if we can show that each $\vy_i$ is an affine function of $\vx$, then it follows that $\vy$ is an affine function of $\vx$.

  It suffices to show that $L'_m$ is a subset of a $k$-dimensional hyperplane.
  This is true if at most $k$ of the $\vu^1,\ldots,\vu^p$ are linearly independent.
  Suppose not; then there are $k+1$ linearly independent vectors among the list.
  Assume without loss of generality that they are $\vu^1,\ldots,\vu^{k+1}$.
  For each $1 \leq i \leq k+1$, let $\vv^i$ be $\vu^i$ projected onto the first $k$ coordinates.
  Since there are $k+1$ vectors and they are $k$-dimensional, $\vv^1,\ldots,\vv^{k+1}$ must be linearly dependent.
  By Lemma~\ref{lem-dependent-integer-vectors}, there exist two lists of natural numbers $N = (n_1,\ldots,n_{k+1})$ and $M = (m_1,\ldots,m_{k+1})$ such that $N \neq M$ and $\sum_{i=1}^{k+1} n_i \vv^i = \sum_{i=1}^{k+1} m_i \vv^i.$
  Then the points
  $$
    \vz^1 = \vb + \sum_{i=1}^{k+1} n_i \vu^i
    \text{   and   }
    \vz^2 = \vb + \sum_{i=1}^{k+1} m_i \vu^i
  $$
  are in $L'_m$.
  They must have different $y$-coordinates, or else we would have $\vz^1 = \vz^2$ (since their first $k$ coordinates agree), which would contradict the linear independence of $\vu^1,\ldots,\vu^{k+1}$.
  Therefore $L'_m$ does not define the graph of a function since these two identical inputs map to two different outputs, a contradiction.
\qedl\end{proof}



\begin{lem} \label{lem-dependent-integer-vectors}
  Let $\vv^1,\ldots,\vv^t\in\N^k$ be linearly dependent vectors.
  Then there are two lists of natural numbers $N = (n_1,\ldots,n_t)\in\N^t$ and $M = (m_1,\ldots,m_t)\in\N^t$ such that $N \neq M$ and $\sum_{i=1}^t n_i \vv^i = \sum_{i=1}^t m_i \vv^i.$
\end{lem}


\begin{proof}
  By the definition of linear dependence, there exist two lists of real numbers $N' = (n'_1,\ldots,n'_t)\in\R^t$ and $M' = (m'_1,\ldots,m'_t)\in\R^t$ such that $N' \neq M'$ and $\sum_{i=1}^t n'_i \vv^i = \sum_{i=1}^t m'_i \vv^i \in \N^k$ (since all points, integer or not, in the basis of $\vv^1,\ldots,\vv^t\in\N^k$ can be so expressed).
  Perhaps some of the coefficients are negative; however, by increasing both $n'_i$ and $m'_i$ by $\min\{n'_i,m'_i\}$ (which changes each sum by the same amount, keeping them equal), we may assume that all coefficients are nonnegative.
  Furthermore, since the sum $\sum_{i=1}^t n_i \vv^i$ is integer-valued, $N',M'\in\Q^t$.

  Let $L$ be the least common multiple of the denominators of each $n'_i$ and $m'_i$ when expressed in lowest terms.
  By multiplying each coefficient by $L$, we obtain nonnegative integers $N = (n_1,\ldots,n_t)\in\N^t$ and $M = (m_1,\ldots,m_t)\in\N^t$ such that $N \neq M$ and $\sum_{i=1}^t n_i \vv^i = \sum_{i=1}^t m_i \vv^i.$
\qedl\end{proof}



\begin{lem} \label{lem-compute-linear-fast}
  Let $f:\N^k\dashrightarrow\N^l$ be a partial affine function.
  Then there is a CRC that computes $f$ on input $\vx$ in expected time $O(\|\vx\| \log \|\vx\|)$, such that the output molecules monotonically increase with time (i.e. none are ever consumed). %, with an exponentially decaying tail.
\end{lem}

\newcommand{\hL}{\widehat{L}}

\begin{proof}
  If $\vy = f(\vx)$, then there exist $kl+l+k$ integers $a_1^1,\ldots,a_k^l\in\Q\cap[0,\infty)$ and $b_1,\ldots,b_l,c_1,\ldots,c_k\in\Z$ such that each $\vy_j = b_j + \sum_{i=1}^k a_i^j (\vx_i + c_i)$.
  Define the CRC as follows.
  It has input species $\Sigma = \{X_1,\ldots,X_k\}$ and output species $\Gamma = \{Y_1,\ldots,Y_l\}$.
  %If $b_j>0$, start with $b_j$ copies of $Y_j$, and otherwise, start with $-b_j$ copies of $K_j$ (``$Y_j$ killer'' molecules).

  Let $b^j_1, \ldots, b^j_k \in \{-|b_j|,\ldots,|b_j|\}$ be integers such that $\sum_{i=1}^k b_i^j = b_j$.
  Let $c_i^1, \ldots, c_i^l \in \{-|c_i|,\ldots,|c_i|\}$ be integers such that $\sum_{j=1}^l c_i^j = c_i$.
  For each $1 \leq i \leq k$ and $1 \leq j \leq l$, start with a leader molecule $\hL_{i,c_i^j}^j$.
  For each $1 \leq i \leq k$ and $1 \leq j \leq l$, let $\frac{n_i^j}{d_i^j}$ be $a_i^j$ expressed as a fraction such that $d_i^j > c_i$ and, if $b_j < 0$, $n_i^j \geq - b_j$.
  For each $1 \leq i \leq k$, add the reaction
  \begin{eqnarray*}
    X_i &\to& X_i^1 + X_i^2 + \ldots + X_i^l
  \end{eqnarray*}
  %For each $1 \leq j \leq l$, add the reaction
%  \begin{equation} \label{rxn-KY}
%    K_j + Y_j \to \emptyset
%  \end{equation}
For each $1 \leq i \leq k$,
%if $c_i > 0$,
$1 \leq j \leq l$ and $m$ such that $\min\{0,c_i^j\} \leq m \leq d_i^j$, add the reactions
\begin{eqnarray*}
    \hL_{i,m}^j + X_i^j &\to& \left\{
                              \begin{array}{ll}
                                \hL_{i,m+1}^j, & \hbox{if $m < d_i^j$;} \\
                                L_{i,0}^j + (n_i^j + b_i^j) Y_j, & \hbox{otherwise.}
                              \end{array}
                            \right.
    \\
    L_{i,m}^j + X_i^j &\to& \left\{
                              \begin{array}{ll}
                                L_{i,m+1}^j, & \hbox{if $m < d_i^j$;} \\
                                L_{i,0}^j + n_i^j Y_j, & \hbox{otherwise.}
                              \end{array}
                            \right.
\end{eqnarray*}

%TODO: explain why it works
  Each initial leader $\hL$ starts counting ($m$ is the ``current count'') at an initial value either above or below 0 (depending on the sign of $c_i$) to account for the initial offset $c_i$ of $X_i$.
  Also, each initial leader releases a different amount of $Y_j$ (again depending on the sign of $b_j$) to account for the initial offset $b_j$ of $Y_j$.
  After counting to $d_i^j$, each initial leader $\hL$ converts to a normal leader $L$, which releases $n_i^j$ $Y_j$ molecules for every $d_i^j$ $X_i$ molecules encountered.
  Therefore (after accounting for initial offsets) each $X_i$ molecule converts into a number of $Y_j$ molecules based on the weighted sum of the $a_i^j$ coefficients.
  Therefore when all $X_i^j$ molecules are consumed, the number of $Y_j$ molecules is the proper value $\vy_j = b_j + \sum_{i=1}^k a_i^j (\vx_i + c_i)$.

  It remains to analyze the expected completion time.
  Let $n = \|\vx\|$.
  Since the total number of molecules in solution at any time is $O(n)$, the volume required is also $O(n)$.
  We measure the time to consume all $X_i$ molecules for all $i$.
  We start with $n$ such molecules, so the time for all of them to convert is the maximum of $n$ exponential random variables, each with constant expected value, which is $O(\log n)$.

  Then all $L_i^j$ molecules must encounter every $X_i^j$ molecule.
  By a coupon collector argument, this requires at most $O(n \log n)$ time.
  Therefore the CRC stabilizes in expected time $O(n \log n)$.
  %TODO: justify exponentially decaying tail
\qedl\end{proof}
}

\opt{normal}{\proofTechnicalLemmas}



==> prelim.tex <==
\section{Preliminaries}
\label{sec-prelim}

Throughout the paper we use both superscripts and subscripts to index variables to make for easier reading; the superscript never means exponentiation.
Apologies in advance.

Given a vector $\vx\in\N^k$, let $\|\vx\| = \|\vx\|_1 = \sum_{i=1}^k |\vx_i|$, where $\vx_i$ denotes the $i$th coordinate of $\vx$.
If $f:\N^k\to\N^l$ is a function, define the \emph{graph} of $f$ to be the set
$\setl{ (\vx,\vy) \in \N^k \times \N^l }{ f(\vx) = \vy }.$
A set $A \subseteq \N^k$ is \emph{linear} if there exist vectors $\vec{b},\vec{u}^1,\ldots,\vec{u}^p \in\N^k$ such that 
$$A=\setl{\vec{b} + n_1 \vec{u}^1 + \ldots + n_p \vec{u}^p}{n_1,\ldots,n_p\in\N}.$$
$A$ is \emph{semilinear} if it is a finite union of linear sets.
We say a partial function $f:\N^k \dashrightarrow \N^l$ is \emph{affine} if there exist $kl$ rational numbers $a_1^1,\ldots,a_k^l\in\Q\cap[0,\infty)$ and $l+k$ integers $b_1,\ldots,b_l,c_1,\ldots,c_k\in\Z$ such that for each $1 \leq j \leq l$, $\vy_j = b_j + \sum_{i=1}^k a_i^j (\vx_i + c_i)$.
%(We use partial functions since evaluating an affine function on integer coordinates may result in a noninteger output.)
%there exist $b,w_1,\ldots,w_k\in\N$ such that if $\vy_j$ is the $j$th coordinate of $f(\vx)$, then $\vy_j = b + \sum_{i=1}^k w_i \vx_i$.
In other words, the graph of $f$, when projected onto the $(k+1)$-dimensional space defined by the $k$ coordinates corresponding to $\vx$ and the single coordinate corresponding to $\vy_j$, is a subset of a $k$-dimensional hyperplane.

%We write $\Z$, $\Z^+$, and $\N$ to denote the set of integers, positive integers, and nonnegative integers, respectively.


%\begin{definition}
%  Let $f,g:\N\to\N$.
%  We say that $f$ is \emph{stably reducible} to $g$, written $f \leqs g$ if ???
%\end{definition}

\subsection{Chemical reaction networks}

If $\Lambda$ is a finite set (in this paper, of chemical species), we write $\N^\Lambda$ to denote the set of functions $f:\Lambda \to \N$.
Equivalently, we view an element $C\in\N^\Lambda$ as a vector of $|\Lambda|$ nonnegative integers, with each coordinate ``labeled'' by an element of $\Lambda$.
Given $X\in \Lambda$ and $C \in \N^\Lambda$, we refer to $C(X)$ as the \emph{count of $X$ in $C$}.
%We also equivalently view an element $C \in \N^\Lambda$ as a \emph{multiset} of elements of $\Lambda$, where $C(X)$ is the multiplicity of element $X \in \Lambda$.
%We therefore write $C \subseteq C'$ to denote that $C(X) \leq C'(X)$ for all $X \in \Lambda$.
We write $C \leq C'$ to denote that $C(X) \leq C'(X)$ for all $X \in \Lambda$.
Given $C,C' \in \N^\Lambda$, we define the vector component-wise operations of addition $C+C'$, subtraction $C-C'$, and scalar multiplication $n C$ for $n \in \N$.
If $\Delta \subset \Lambda$, we view a vector $C \in \N^\Delta$ equivalently as a vector $C \in \N^\Lambda$ by assuming $C(X)=0$ for all $X \in \Lambda \setminus \Delta.$


Given a finite set of chemical species $\Lambda$, a \emph{reaction} over $\Lambda$ is a triple $\alpha = \langle \bfr,\bfp,k \rangle \in \N^\Lambda \times \N^\Lambda \times \R^+$, specifying the stoichiometry of the reactants and products, respectively, and the \emph{rate constant} $k$.
If not specified, assume that $k=1$ (this is the case for all reactions in this paper), so that the reaction $\alpha=\langle \bfr,\bfp,1 \rangle$ is also represented by the pair $\pair{\bfr}{\bfp}.$
For instance, given $\Lambda=\{A,B,C\}$, the reaction $A+2B \to A+3C$ is the pair $\pair{(1,2,0)}{(1,0,3)}.$
A \emph{(finite) chemical reaction network (CRN)} is a pair $N=(\Lambda,R)$, where $\Lambda$ is a finite set of chemical \emph{species},
%$\Sigma \subseteq \Lambda$ be a finite \emph{input alphabet} (a.k.a., \emph{set of input species}), $\phi:\Lambda\to\{0,1\}$ is the \emph{output function},
and $R$ is a finite set of reactions over $\Lambda$.
A \emph{configuration} of a CRN $N=(\Lambda,R)$ is a vector $C \in \N^\Lambda$.
We also write $\#_C X$ to denote $C(X)$, the \emph{count} of species $X$ in configuration $C$, or simply $\# X$ when $C$ is clear from context.


Given a configuration $C$ and reaction $\alpha=\pair{\bfr}{\bfp}$, we say that $\alpha$ is \emph{applicable} to $C$ if $\bfr \leq C$ (i.e., $C$ contains enough of each of the reactants for the reaction to occur).
If $\alpha$ is applicable to $C$, then write $\alpha(C)$ to denote the configuration $C + \bfp - \bfr$ (i.e., the configuration that results from applying reaction $\alpha$ to $C$).
If $C'=\alpha(C)$ for some reaction $\alpha \in R$, we write $C \to_N C'$, or merely $C \to C'$ when $N$ is clear from context.
An \emph{execution} (a.k.a., \emph{execution sequence}) $\calE$ is a finite or infinite sequence of one or more configurations $\calE = (C_0, C_1, C_2, \ldots)$ such that, for all $i \in \{1,\ldots,|\calE|-1\}$, $C_{i-1} \to C_{i}$.
If a finite execution sequence starts with $C$ and ends with $C'$, we write $C \to_N^* C'$, or merely $C \to^* C'$ when the CRN $N$ is clear from context.
In this case, we say that $C'$ is \emph{reachable} from $C$.

Let $\Delta \subseteq \Lambda$.
We say that $P\in\N^{\Delta}$ is a \emph{partial configuration (with respect to $\Delta$)}.
We write $P = C \rest \Delta$ for any configuration $C$ such that $C(X)=P(X)$ for all $X \in \Delta$, and we say that $P$ is the \emph{restriction of $C$ to $\Delta$}.
%Define the \emph{partial configuration $C$ with respect to $\Delta\subseteq \Lambda$}, written $C \rest \Delta \in \N^\Delta$, to be such that $(C \rest \Delta)(X) = C(X)$ for all $X \in \Delta$.
%We say $C \rest \Delta$ is a \emph{partial configuration}.
Say that a partial configuration $P$ with respect to $\Delta$ is \emph{reachable} from configuration $C'$ if there is a configuration $C$ reachable from $C'$ and $P = C \rest \Delta$.
In this case, we write $C' \to^* P$.

An infinite execution $\calE = (C_0,C_1,C_2,\ldots)$ is \emph{fair} if, for all partial configurations $P$, if $P$ is infinitely often reachable then it is infinitely often reached.\footnote{i.e.
$(\forall \Delta \subseteq \Lambda) (\forall P\in\N^\Delta) [((\exists^\infty i\in\N)\ C_i \to^* P) \implies ((\exists^\infty j\in\N)\ P = C_j \rest \Delta)].$}
In other words, no reachable partial configuration is ``starved''.
This definition of fairness is stricter than that used by Angluin, Aspnes, and Eisenstat~\cite{AngluinAE06}, which used only full configurations rather than partial configurations.
We choose this definition to prevent intuitively unfair executions from vacuously satisfying the definition of ``fair'' simply because of some species whose count is monotonically increasing with time (preventing any configuration from being infinitely often reachable).\footnote{Such a definition is unnecessary in the work of Angluin, Aspnes, and Eisenstat~\cite{AngluinAE06} because population protocols by definition have a finite state space, since they enforce that every reaction has precisely two reactants and two products.}

Note that the definition given above, applied to finite executions, deems all of them fair vacuously.
We wish to distinguish between finite executions that can be extended by applying another reaction and those that cannot.
Say that a configuration is \emph{terminal} if no reaction is applicable to it.
%A finite execution is \emph{terminal} if it ends in a terminal configuration.
We say that a finite execution is \emph{fair} if and only if it %is terminal.
ends in a terminal configuration.

%TODO: mention that this is different from Aspnes because they use the "null" reaction



In order to show that CRNs can compute semilinear functions, we need to have some guarantee that the execution sequence is not chosen such that some reactions are simply not allowed to happen.
(For example, $\{X \to 2Y, A \to B, B \to A\}$ cannot correctly compute $y = 2x$ if an ``adversary'' simply does not let the first reaction occur, always preferring the second or third.)
We consider two models.
In the first part of this paper, we follow~\cite{AngluinAE06} in applying  the above condition of fairness on the allowed execution sequences, which captures combinatorially what we need of the execution sequence.
In the second part of the paper (Section~\ref{sec:detfuncspeed}) we consider the  kinetic model, which ascribes probabilities  to execution sequences.
The kinetic model also defines the time of reactions, allowing us to study the computational complexity of the CRN computation.
Note that in the kinetic model, if the reachable configuration space is bounded for any start configuration (i.e.\ if from any starting configuration there are finitely many configurations reachable) then any observed execution sequence will be fair with probability 1.
(This will be the case for our construction in Section~\ref{sec:detfuncspeed}.)













\subsection{Stable decidability of predicates} \label{subsec-prelim-pred}
We now review the definition of stable decidability of predicates introduced by Angluin, Aspnes, and Eisenstat~\cite{AngluinAE06}.
Those authors use the term ``stably \emph{compute}'', but we reserve the term ``compute'' to apply to the computation of non-Boolean functions.
Intuitively, some species ``vote'' for a yes/no answer, and a CRN $N$ is a stable decider if, for all initial configurations, $N$ is guaranteed (under fair executions) to reach a consensus vote, which is potentially different for different initial configurations but consistent over all fair executions starting from a fixed initial configuration.

A \emph{chemical reaction decider} (CRD) is a tuple $\calD=(\Lambda,R,\Sigma,\Upsilon,\phi,\sigma)$, where $(\Lambda,R)$ is a CRN, $\Sigma \subseteq \Lambda$ is the \emph{set of input species}, $\Upsilon \subseteq \Lambda$ is the set of \emph{voters}, $\phi:\Upsilon\to\{0,1\}$ is the \emph{(Boolean) output function}, and $\sigma \in \N^{\Lambda \setminus \Sigma}$ is the \emph{initial context}.
Intuitively, the goal is for the CRD to get all voters to be eventually unanimous and correct (and for at least one to be present).
An input to $\calD$ will be a vector $I_0\in\N^\Sigma$.
Thus a CRD together with an input vector defines an initial configuration $I$ defined by $I(X) = I_0(X)$ if $X \in \Sigma$, and $I(X) = \sigma(X)$ otherwise.
We say that such a configuration is a \emph{valid initial configuration}, i.e., $I \rest (\Lambda \setminus \Sigma) = \sigma$.
%\footnote{The difference between $\Lambda$ and $\Sigma$ is analogous to the difference between an input alphabet and a tape alphabet of a Turing machine. However, due to the CRN's lack of ``positional information'' that allows a Turing machine to represent a symbol $a \in \Gamma$ as a string $x \in \Sigma$ for $\Sigma \subsetneq \Gamma$, extra species are a necessity rather than merely a convenience for performing certain computations.}
If we are discussing a CRN understood from context to have a certain initial configuration $I$, we write $\#_0 X$ to denote $I(X)$.

%Similarly, given a finite output alphabet $\Gamma$, an \emph{output function} is a function $\phi:\Lambda\to\Gamma$.
%In this paper, we always choose $\Gamma=\{0,1\}$, so we may equivalently view $\Gamma$ as a partition of $\Lambda$ into two disjoint subsets $\Lambda_0 = \setr{X\in \Lambda}{\phi(X)=0}$ and $\Lambda_1 = \setr{X\in \Lambda}{\phi(X)=1}$.
%For brevity we often take $\Gamma$ to be a partition of $\Lambda$, and take $\phi(X)$ to be the symbol associated as the input function.

%Let $\phi:\Lambda\to\{0,1\}$ be a \emph{(Boolean) output function} for the CRN $N=(\Lambda,\Sigma,R)$.
We extend $\phi$ to a partial function $\Phi:\N^\Lambda \dashrightarrow \{0,1\}$ as follows.
$\Phi(C)$ is undefined if either $C(X) = 0$ for all $X \in \Upsilon$, or if there exist $X_0,X_1 \in \Upsilon$ such that $C(X_0) > 0$, $C(X_1) > 0$, $\phi(X_0)=0$ and $\phi(X_1)=1$.
Otherwise, there exists $b\in\{0,1\}$ such that $(\forall X \in \Upsilon) (C(X)>0 \implies \phi(X)=b)$; in this case, the \emph{output} $\Phi(C)$ of configuration $C$ is $b$.

A configuration $C$ is \emph{output stable} if $\Phi(C)$ is defined and, for all $C'$ such that $C \to^* C'$, $\Phi(C') = \Phi(C)$.
We say that a CRD $\calD$ is \emph{stable} if, for any valid initial configuration $I \in \N^\Lambda$, there exists $b\in\{0,1\}$ such that \emph{every} fair execution $\calE = (I, C_1, C_2, \ldots)$ contains an output stable configuration $C$ with $\Phi(C)=b$ (i.e., $\calD$ always converges to a defined output on input $I$, and this output is the same for any fair execution starting from $I$).
If $\calD$ is stable, then some unique subset $S_0 \subseteq \N^\Sigma$ of all possible initial configurations always converges to output 0 and stays with that output, and the remainder $S_1 = \N^\Sigma \setminus S_0$ always converges to output 1 and stays with that output.
We say that $\calD$ \emph{stably decides} the set $S_1$, or that $\calD$ \emph{stably decides} the predicate $\psi:\N^\Sigma \to \{0,1\}$ defined by $\psi(I_0) = 1$ if $I_0 \in S_1$ and $\psi(I_0) = 0$ if $I_0 \in S_0$.

%A set $A \subseteq \N^k$ is \emph{linear} if there exist vectors $\vec{b},\vec{u}^1,\ldots,\vec{u}^p \in\N^k$ such that 
%\begin{equation}  \label{eq:semilinear}
%A=\setl{\vec{b} + n_1 \vec{u}^1 + \ldots + n_p \vec{u}^p}{n_1,\ldots,n_p\in\N}.
%\end{equation}
%$A$ is \emph{semilinear} if it is a finite union of linear sets.

%  \item Semilinear sets are \emph{very simple} computationally and logically:
%    \begin{enumerate}
%      \item $=$ sets definable in Presburger arithmetic (theory of natural numbers with addition but no multiplication)
%
%      \item $=$ sets decidable by \emph{reversal-bounded counter machines}: finite state machines with a finite set of registers that can be incremented, decremented, or tested for 0, and each may only switch from incrementing to decrementing once.
%    \end{enumerate}

The following theorem is due to Angluin, Aspenes, and Eisenstat~\cite{AngluinAE06}:

\begin{theorem}[\cite{AngluinAE06}] \label{thm-semilinear}
A set $A \subseteq \N^k$ is stably decidable by a CRD if and only if it is semilinear.
\end{theorem}

%In fact, the forward direction of Theorem~\ref{thm-semilinear} (every stably decidable set is semilinear) holds even if stable computation is defined with respect to \emph{any} relation $\to^*$ on $\N^k$ that is reflexive, transitive, and ``respects addition'' [$(\forall C_1,C_2,X\in\N^k)\ (C_1 \to^* C_2) \implies (C_1 + X \to^* C_2 + X$)].
%These properties can easily be shown to hold for the CRN reachability relation.
%The third property, in particular, means that if some molecules $C_1$ can react to form molecules $C_2$, then it is possible for them to react in the presence of some extra molecules $X$, such that no molecules from $X$ react at all.

The definitions of~\cite{AngluinAE06} assume that $\Upsilon = \Lambda$ (i.e., every species votes).
However, it is not hard to show that we may assume there are only two voting species, $L^0$ and $L^1$, so that $\# L^0 > 0$ and $\# L^1 = 0$ means that the CRD is answering ``no'', and $\# L^0 = 0$ and $\# L^1 > 0$ means that the CRD is answering ``yes.''
This convention will be more convenient in this paper.










\subsection{Stable computation of functions}

%TODO: add note that the extension from Boolean predicates to functions described by Aspnes and Ruppert applies only to finite-range functions, where one can choose $|\Lambda| \geq |Y|$ for output range $Y$.




We now define a notion of stable computation of \emph{functions} similar to those above for predicates.\footnote{The extension from Boolean predicates to functions described by Aspnes and Ruppert~\cite{aspnes2007introduction} applies only to finite-range functions, where one can choose $|\Lambda| \geq |Y|$ for output range $Y$.}
Intuitively, the inputs to the function are the initial counts of inputs species $X_1,\ldots,X_k$, and the outputs are the counts of ``output" species $Y_1,\ldots,Y_l$, such that the CRN is guaranteed to eventually reach a configuration in which the counts of the output species have the correct values and never change from that point on.
%For example, the CRN $N$ with the single reaction $X \to 2Y$ computes the function $f(n)=2n$ in the sense that, if $N$ starts in an initial configuration with $n$ copies of $X$ and 0 copies of $Y$, then $N$ is guaranteed to stabilize to a configuration with $2n$ copies of $Y$ (and no copies of $X$).
%Similarly, the function $f(n) = \floor{n/2}$ is computed by the single reaction $2X \to Y$, in that the final configuration is guaranteed to have exactly $\floor{n/2}$ copies of $Y$ (and 0 or 1 copies of $X$, depending on whether $n$ is even or odd).

We now formally define what it means for a CRN to stably compute a function.
Let $k,l\in\Z^+$.
A \emph{chemical reaction computer (CRC)} is a tuple $\calC=(\Lambda,R,\Sigma,\Gamma,\sigma)$, where $(\Lambda,R)$ is a CRN, $\Sigma \subset \Lambda$ is the \emph{set of input species}, $\Gamma \subset \Lambda$ is the \emph{set of output species}, such that $\Sigma \cap \Gamma = \emptyset$, $|\Sigma|=k$, $|\Gamma|=l$, and $\sigma \in \N^{\Lambda\setminus\Sigma}$ is the \emph{initial context}.
Write $\Sigma = \{X_1,X_2,\ldots,X_k\}$ and $\Gamma = \{Y_1,Y_2,\ldots,Y_l\}$.
We say that a configuration $C$ is \emph{output count stable} if, for every $C'$ such that $C \to^* C'$ and every $Y_i \in \Gamma$, $C(Y_i) = C'(Y_i)$ (i.e., the counts of species in $\Gamma$ will never change if $C$ is reached).
As with CRD's, we require initial configurations $I$ of $\calC$ with input $I_0\in\N^\Sigma$ to obey $I(X)=I_0(X)$ if $X\in\Sigma$ and $I(X)=\sigma(X)$ otherwise, calling them \emph{valid initial configurations}.
We say that $\calC$ \emph{stably computes} $f:\N^k\to\N^l$ if, for every valid initial configuration $I \in \N^{\Lambda}$, every fair execution $\calE = (I,C_1,C_2,\ldots)$ contains an output count stable configuration $C$ such that $f(I(X_1), I(X_2), \ldots, I(X_k)) = (C(Y_1), C(Y_2), \ldots, C(Y_l))$.
In other words, the counts of species in $\Gamma$ are guaranteed to converge to the value of $f(x_1,x_2,\ldots,x_k)$ when started in an initial configuration with $x_i$ copies of $X_i$ for each $i \in \{1,\ldots,k\}$. % and no copies of any species outside of $\Sigma$.
We say that such a CRC is \emph{count stable}.
For any species $A \in \Lambda$, we write $\#_\infty A$ to denote the eventual convergent count of $A$ if $\# A$ is guaranteed to stabilize; otherwise, $\#_\infty A$ is undefined.
%TODO: make a cleaner definition of $\#_\infty$

As an example of a formally defined CRC consider the function $f(x) =   \floor{x/2}$ shown in Fig.~\ref{fig:examples}(a). 
This function is deterministically computed by the CRC $(\Lambda,R,\Sigma,\Gamma,\sigma)$ where $(\Lambda,R)$ is the CRN consisting of a single reaction $2 X \to Y$, $\Sigma = \{X\}$ is the set of inputs species, $\Gamma = \{Y\}$ is the set of output species, and the initial context $\sigma$ is zero for all species in $\Lambda\setminus\Sigma$.
In Fig.~\ref{fig:examples}(b) the initial context $\sigma(N)=1$, and is zero for all other species in in $\Lambda\setminus\Sigma$.

In sections~\ref{sec:detfunc} and \ref{sec:detfuncspeed} we will describe systematic (but much more complex) constructions for these and all functions with semilinear graphs.









\subsection{Kinetic model}

In this paper, the rate constants of all reactions are $1$, and we define the kinetic model with this assumption. 
A reaction is \emph{unimolecular} if it has one reactant and \emph{bimolecular} if it has two reactants.
We use no higher-order reactions in this paper when using the kinetic model.

The kinetics of a CRN is described by a continuous-time Markov process as follows.
Given a fixed volume $v$ and current configuration $C$, the \emph{propensity} of a unimolecular reaction $\alpha : X \to \ldots$ in configuration $C$ is $\rho(C, \alpha) = \#_C X$.
The propensity of a bimolecular reaction $\alpha : X + Y \to \ldots$, where $X \neq Y$, is $\rho(C, \alpha) = \frac{\#_C X \#_C Y}{v}$.
The propensity of a bimolecular reaction $\alpha : X + X \to \ldots$ is $\rho(C, \alpha) = \frac{1}{2} \frac{\#_C X (\#_C X - 1)}{v}$.
The propensity function determines the evolution of the system as follows.
%If the system is in configuration $C$, no further reactions are possible if no reaction is applicable.
%Otherwise,
The time until the next reaction occurs is an exponential random variable with rate $\rho(C) = \sum_{\alpha \in R} \rho(C,\alpha)$ (note that $\rho(C)=0$ if no reactions are applicable to $C$).
The probability that next reaction will be a particular $\alpha_{\text{next}}$ is $\frac{\rho(C,\alpha_{\text{next}})}{\rho(C)}$.

The kinetic model is based on the physical assumption of well-mixedness valid in a dilute solution.
Thus, we assume the \emph{finite density constraint}, which stipulates that a volume required to execute a CRN must be proportional to the maximum molecular count obtained during execution~\cite{SolCooWinBru08}.
In other words, the total concentration (molecular count per volume) is bounded.
This realistically constrains the speed of the computation achievable by CRNs.
Note, however, that it is problematic to define the kinetic model for CRNs in which the reachable configuration space is unbounded for some start configurations, because this means that arbitrarily large molecular counts are reachable.\footnote{One possibility is to have a ``dynamically" growing volume as in~\cite{SolCooWinBru08}.}
We apply the kinetic model only to CRNs with  configuration spaces that are bounded for each start configuration.




==> pthsa.tex <==
\input{main}

==> results.tex <==
\section{Results}
\label{sec-results}

\input{func}

\input{func-speed}

%We first establish some results that will allow for simpler protocols later.
%Some of these results are implicit in~\cite{angluin2007computational}, but we provide proofs here to make the paper self-contained.
%
%We first note that any function stably computable with the help of a ``leader'' can be stably computed without a leader by performing leader election in conjunction with the function computation.
%
%Formally, say that a CRC $\calC=(\Lambda,R,\Sigma,\Gamma)$ stably computes a function $f:\N^k\to\N^l$ \emph{with a leader} if there is a species $L \in \Lambda \setminus \Sigma$ such that, for any initial configuration $I \in \N^{\Sigma \cup \{L\}}$ such that $I(L) = 1$, $\calC$ stably computes $f$.
%Say that a CRN $\calC=(\Lambda,R,\Sigma,\Gamma)$ stably computes a function $f:\N^k\to\N^l$ \emph{with multiple leaders} if there is a species $L \in \Lambda \setminus \Sigma$ such that, for any initial configuration $I \in \N^{\Sigma \cup \{L\}}$ such that $I(L) > 0$, $\calC$ stably computes $f$.
%TODO: define this formally
%
%\begin{lemma}
%  A function $f:\N^k\to\N^l$ is stably computable with a leader if and only if it is stably computable with multiple leaders.
%\end{lemma}
%
%\begin{proof}
%  If $f$ is stably computable with multiple leaders, then it is trivially computable with a single leader.
%  To show the converse, let $N=(\Lambda,\Sigma,R)$ be a CRN that stably computes $f$ with a leader $L$.
%  Define the CRN $N'=(\Lambda',\Sigma,R')$ as follows.
%  Let $\Lambda' = \Lambda \cup \{NL\}$, and let $R' = R \cup \{\alpha\}$, where $\alpha$ is the reaction $L + L \to L + NL$.
%
%  TODO: finish this
%\end{proof}
%
%\begin{lemma}
%  Every function stably computable with a leader is stably computable without a leader.
%\end{lemma}
%
%\begin{proof}
%  Let $N=(\Lambda,\Sigma,R)$ be a CRN that stably computes $f$ with a leader $L$.
%  Define the CRN $N'=(\Lambda',\Sigma',R')$ as follows.
%  For each $X \in \Sigma$, let $X' \in \Sigma'$, and for each $X,Y\in\Sigma$, add the reaction $f$.
%
%  TODO: finish this
%\end{proof}
%
%
%
%We show an alternative
%
%\begin{lemma}
%
%\end{lemma}
%
%
%TODO: show that sometimes it is necessary to allow configurations to keep changing even if they are output-stable or count-stable, or that we can always reach a configuration in which no reactions are possible
%
%TODO: prove some lemmas about whether it is necessary to have a leader (when computing both functions and predicates), and whether it is necessary when computing functions to have extra species left over that are not output species
%
%TODO: show that we can remove the requirement that output species be disjoint from input species

%The following lemma shows that we can execute a ``dynamic comparison'' between the counts of two species whose counts changing before they stabilize, but only by monotonic increase.
%
%\begin{lemma}
%  Let $N$ be a CRN, and let $A$ and $B$ be two species in $N$
%\end{lemma}




